How People Prompt to Create Interactive VR Scenes

Generative AI tools can provide people with the ability to create virtual environments and scenes with natural language prompts. Yet, how people will formulate such prompts is unclear -- particularly when they inhabit the environment that they are designing. For instance, it is likely that a person might say, "Put a chair here", while pointing at a location. If such linguistic features are common to people's prompts, we need to tune models to accommodate them. In this work, we present a wizard-of-oz elicitation study with 22 participants, where we studied people's implicit expectations when verbally prompting such programming agents to create interactive VR scenes. Our findings show that people prompt with several implicit expectations: (1) that agents have an embodied knowledge of the environment; (2) that agents understand embodied prompts by users; (3) that the agents can recall previous states of the scene and the conversation, and that (4) agents have a commonsense understanding of objects in the scene. Further, we found that participants prompt differently when they are prompting in situ (i.e. within the VR environment) versus ex situ (i.e. viewing the VR environment from the outside). To explore how our could be applied, we designed and built Oastaad, a conversational programming agent that allows non-programmers to design interactive VR experiences that they inhabit. Based on these explorations, we outline new opportunities and challenges for conversational programming agents that create VR environments.

==> archive/old-04-user-experience-study.tex <==
\section{User Experience Study}

Our goal in designing and developing MAGIC was to explore the experience of conversational prototyping in the hands of non-programmers. To this end, we designed a user experience study where participants used MAGIC as a design probe: first, to understand the extent to which MAGIC enabled an effective and enjoyable creation experience for non-programmers; second, to explore and understand the nature of conversational prototyping---what aspects of the conversational interaction are ineffective and need to be better supported?

We designed a four part design study, where we asked participants create interactive experiences with MAGIC---first beginning with carefully scripted prompts that were sure to work, progressively allowing participants more flexibility in crafting their prompts until they we were ultimately asking them craft prompts that were clearly beyond the capacity of the system. Throughout this process, the goal was to carefully study how they used MAGIC conversationally, and to capture ways in which they \emph{expected} to interact with MAGIC. 

\paragraph{Participants.} We recruited...

\paragraph{Procedure.} The one-hour study was divided into four phases, with the beginning phases carefully scripted all the way to fully unscripted creative final phase.

\begin{description}
    \item [Phase 1: Tutorial] The goal of the first phase was to give participants an understanding of how the system functioned, much as one would use a system at a system demonstration. To this end, the experience was slowly paced, and participants' utterances were scripted in advance for them to read. Participants donned the VR headset, and the basic function of the system explained to them. In the VR environment, a scripted billboard appeared in the virtual environment for participants to follow along and read. This billboard explained how they could dictate a prompt, and then explained that the system would create a VR experience based on this prompt. They were then told how to instantiate two different experiences \texttt{Prompt: Create a lamp that turns on when I touch it, and turns off when I touch it again}, and \texttt{Prompt: Put LED lights on the walls. When I get near them, turn them on}. Once each of these experiences were successfully created, participants were told that they could use slight variations on the prompts, where the system would still create the same system.

    \item [Phase 2: Simple Systems] The goal of the second phase was to allow participants more flexibility in generating prompts, though the \emph{idea} of the system would be provided to them. To this end, we used the billboard in the virtual world to show videos of example systems that we wanted participants to build. Here, these videos were all of systems that had previously been created in MAGIC, so they were possible with the system. We showed participants a set of three such systems, and allowed participants to watch the videos over as many times as they liked. Then, when they indicated they were ready, we allowed them to attempt to create the same experience using verbal prompts of their choosing. Participants were allowed to make multiple attempts---the idea intention was to allow them to explore how to phrase and use language to create the intended systems.
    
    \item [Phase 3: Complex Systems] Our goal here was to ask participants to create approximations of interactive experiences we drew from the outside world. These videos included a theme park experience, a museum experience, and a research prototype. In each of these cases, it was not possible to recreate from scratch the entirety of the experience, but we asked participants to consider a part of the experience, and to try to recreate it with MAGIC. In each case, we gave participants 5 minutes with each video to recreate parts of the experience.

    % TODO: Alternately, maybe this could be "free play" time. The difference to me is not huge.
    \item [Phase 4: Brainstorming] In this phase, participants removed the VR headset, and were asked to brainstorm and dream up interactive experiences. We asked them to sketch out these interactive experiences, explaining them to us. Then, we asked them to speak aloud, as if to MAGIC, to create the system. We allowed them as many attempts as they wanted to do this.
    
\end{description}

\paragraph{Data Collection.} We recorded ...




==> figures/api.tex <==

% Using something from here: https://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell

% TODO:
% - format header nicer
% - top align the major cells
% - left align the content

\begin{table}
    \centering
    \begin{tabular}{lll}
        \hline
        \thead{Objects}  & \thead{Properties} & \thead{Interactions} \\
        \hline
        \makecell{Desk lamp \\ Floor lamp \\ LED light \\ Office chair \\ Office desk } & \makecell{Position \\ Orientation \\ Size \\ Height \\ Width \\ Colour } & \makecell{ LookingAt \\ PointingAt \\ DistanceFromUser}\\
        \hline
    \end{tabular}
    \caption{MAGIC currently provides several pre-defined objects that can be instantiated into the scene. Each of these objects carries several common properties, while some specific objects have properties unique to them. Finally, the system can recognize various types of user interactions with these objects.}
    \label{tab:api}
\end{table}

==> figures/user-experience.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/images/interaction schematic.png}
  \caption{MAGIC allows users to specify the function of the interactive system verbally in VR. Through text, it provides the user with an understanding of how it understood the prompt, and then in the VR space, creates the system that the user described.}
  \Description{}
  \label{fig:user-experience}
\end{figure}

==> sections/99-AWARD_WINNING_TEXT.tex <==
00 title and abstract.tex
%\title{Creating Interactive VR Experiences with In-Situ and Ex-Situ Prompts}
%\title{Challenges of Describing Interactive Behaviour with a Conversational Programming Agent}
%\title{Toward Conversational Prototyping: Assisting Non-Programmers to Prototype Interactive Spaces}
% Specifying Behaviour of Interactive Spaces through Conversation
% Conversational Prototyping of Interactive Spaces
% Limitations of Single Turn Specification of Interactive Spaces

% go at this from the conversational/generative AI programming angle
% or go at this from the IoT prototyping angle?


%Generative AI tools show promise in helping programmers to prepare code under well-specified conditions. 
%Yet, it is unclear how to design effective generative AI tools for non-programmers to envision and prototype interactive spaces.
%We present MAGIC, an interactive system that allows non-programmers to create interactive VR experiences through a conversational interface.
%Using MAGIC as a design probe with non-programmers, we explored how non-programmers would specify interactive system behaviour through conversation.
%We found that non-programmers needed multiple opportunities to articulate and refine their ideas, and that these ideas are described with proxemic and deicitic references that need to be accounted for in conversational prototyping systems.

% Creating and prototyping virtual scenes is possible with conversational programming agents
% We explore the user experiences that are enabled by such conversational programming agents, and outline user experience challenges that need to be overcome: first by building our own conversational programming agent, and second by eliciting scene descriptions from people that they would use such a conversational programming agent with
% We find that prompts elicited in an embodied context tend to rely implicitly on embodied factors such as gaze or body position.
% We find that in terms of descriptive complexity, prompts that instantiate or manipulate scene objects tend to have lower variation compared to prompts that suggest interactive behaviour.
% Furthermore, that interactive behaviours are challenging to describe for most participants, where they expect to be able to refine the scene that they see, rather than regenerating the entire scene.


% MAking Generation Interactive and Captivating


01 introduction.tex

%Among these tools are diffusion models, a class of generative models that employ a diffusion process to iteratively transform a simple noise distribution into complex data distribution. Such models excel in synthesizing high-quality and diverse images, providing  creatives with control over various aspects of the generation process, such as style, content, and stochasticity---often with natural language prompts---ultimately expanding the possibilities for artistic expression and content creation.

% Maybe talk about why elicitation vs having a real system. Maybe less of a problem for DIS

% Briefly, participants are exposed to two scenes---a ``before'' scene and an ``after'' scene (each called a referent), and asked to explain how they would communicate with a programming agent to get from the ``before'' scene to the ``after'' scene.

%While Oastaad relies on a general purpose large language model (OpenAI GPT), giving users considerable flexibility in crafting their prompts, anecdotally, we found that there were still many prompts that it did not handle well.

%- In this work, we first constructed Ostaad, a conversational agent that enables people to use embodied voice prompts to construct VR scenes.
%Very little research has explored how to create programming agents for non-programmers. The vast majority of work exploring generative program synthesis has focused on enhancing programmer productivity. Such tools show promise in helping programmers to prepare code under well-specified conditions. XXx demonstrate how it can be used inline with coding IDEs to generate code based on a prompt and the surrounding code as context. Other advances have shown how these generative AI tools can also assist programmers in understanding programming problems, debugging code, and so forth. Using these generative models to support non-programmers in programming-like tasks has been less well explored. Xxx did such and such, YYyy did such and such. Yet, in general, we expect two major differences between how and when non-programmers vs. programmers will use such models. First, we expect non-programmers to have a harder time articulating non-ambiguous, clear, and well-defined programming problems---this would make it harder for the generative model to produce effective code. Second, we expect non-programmers to { ``write code'' in non-traditional situations }. It is unclear how effective advances in tooling for supporting programmers will be in supporting non-programmers.

%This paper focuses on the iterative design of MAGIC (MAking Generation Interactive and Captivating), which we use as a probe to explore the concept of ``conversational prototyping.'' Conversational prototyping allows people to verbally articulate and describe the function of a computer system declaratively. The programming subsystem then interprets these ideas and intentions, and provides users with a functional prototype that users can use, test, and assess. Our prototype system MAGIC allows people to prototype interactive objects and spaces in VR by verbally describing the idea. MAGIC interprets these ideas within the context of available objects and interactions, and immediately creates the VR experience for the user to experience.


%We then used MAGIC as a design probe with non-programmers to understand aspects of ``conversational prototyping''. Our focus here was on the ways it addressed non-programmers needs, and also the ways in which the conversational interface needed to be improved to fulfill non-programmers' expectations. Our findings here reveal several important directions for conversational programming interfaces that are aimed at non-programmers. First, that particularly with embodied experiences, the conversational interface needs to understand spatial and deictic references. Second, that how people verbally articulate their ideas requires substantial refinement---both \textit{while} they are describing their ideas, as well as once their ideas have been realized; systems need to account for these ``unclean'' prompts. Finally, that ambiguity can be used as a design resource here, where the system can generate multiple candidate prototypes based on the prompt, and that these can be used by the user to refine their thinking.

%This paper makes primarily three contributions. First, we contribute a conversational prototyping system in MAGIC, which allows non-programmers to create interactive VR experiences. Second, we contribute the findings of a design study that explores how non-programmers expect to use conversational interfaces to create interactive experiences. These findings suggest new directions for conversational programming interfaces. Finally, based on these findings, we describe ....

%- Yet, we do not yet have data on *how* people will expect to be able to prompt and create such scenes and environments. Such knowledge will be useful to tune these generative models.
%- In this work, we first constructed Ostaad, a conversational agent that enables people to use embodied voice prompts to construct VR scenes.
%- To study how people would use embodied conversational programming agents like Ostaad, we conducted a two part user study. In the first part of the user study, we asked users to familiarize themselves with the system to create scenes by follow prescribed scripts. In the second part of the user study, we used an elicitation-study type approach, where we deliberately perturbed the results of the agent to understand how users would reformulate their prompts to the system.



%addressing several questions: How easily understood are people's prompts in relation to the environment? Would people's prompts differ if they prompted while inhabiting the environment through VR (\emph{in-situ}) versus designing outside of the environment (\emph{ex-situ})? We might expect that prompts should contain bodily gestures, as they are communicative acts~\cite{fraser_supporting_1999}.

%information addressing several questions we had about how programming agents for 3D interactive scenes might be used: What capabilities do people implicitly have of these programming agents when they prompt them? How do people expect to be able to use their bodies to communicate (e.g. through gesture) their intent with such programming agents?  Such knowledge will be useful in designing interfaces and tuning generative models used to create these environments.

%first, how would participants prompt \textit{in situ} vs. \textit{ex situ}; second, how smoothly would prompts be when articulated verbally; third, how do people refine the design from their prompts, and finally, how do prompts differ when they involve interactive behaviour vs designing scene objects.


02 related work.tex
% Authoring 3D virtual environments and their dynamic behaviors in response to user input has long seen important applications in the creative and engineering industry. 

\begin{comment}
We set the stage for our work by outlining three areas of work: first, efforts to support non-programmers in prototyping, where we outline several principles underpinning these approaches; next, we discuss recent advances in generative AI tools that support programmers in preparing code, and finally, we discuss some explorations of interactive spaces to circumscribe our area of interest in this work.

% This needs to be bounded even more. Maybe explore reordering the sections, too.

\subsection{Helping Non-Programmers Prototype}

Mixing of "teaching people how to code" vs. "helping people to prepare code" vs. "helping people to make computers do things they need"
\end{comment}


Figures

\begin{comment}
\begin{table}[h]
  \centering
  \begin{tabular}{|c|}
    \hline
    \begin{minipage}{0.8\textwidth}
      \begin{itemize}
        \item Animals (dog, cat, horse, elephant, rabbit, etc.)
        \item Office furniture (desk, table, chair, couch, lamp, cabinet, etc.)
        \item Object primitives (cube, sphere, pyramid, etc.)
      \end{itemize}
    \end{minipage} \\
    \hline
  \end{tabular}
  \captionof{table}{Oastaad currently provides users with access to the following objects.}
  \label{tab:programmable-objects}
\end{table}


\begin{table}[h]
  \centering
  \begin{tabular}{|c|}
    \hline
    \begin{minipage}{0.8\textwidth}
      \begin{itemize}
      \item Object creation (i.e. instantiating an object)
      \item Modifying an object (e.g. changing its parameters, such as height, size, orientation, etc.)
      \item Modifying the scene (e.g. moving objects)
      \item Proxemic interaction (e.g. near by, far away, looking at, pointing at, touching)
      \end{itemize}
    \end{minipage} \\
    \hline
  \end{tabular}
  \captionof{table}{Oastaad provides users with many interaction capabilities.}
  \label{tab:programmatic-capabilities}
\end{table}

\end{comment}

Considerable efforts have explored how to support non-programmers to program and develop code.

- programming by demonstration (robotics)

- macros (

- visual programming and code blocks (higher level specification and stringing together) 



\subsection{Supporting Programmers to Write Code using Automation}

Recent efforts based on large language models (LLMs) have produced tools that have been demonstrated to be effective in supporting programmers. These LLMs have been been trained on large quantities of code as well as text, giving the LLMs the ability to generate code snippets, or explain code snippets and error messages based on well-formed user prompts. Commercial products such as GitHub Co-Pilot, for instance, allow for users to prompt the system by providing a comment, where the LLM is then tasked with generating code that provides functionality described in the prompt. Other projects provide side-bars that similarly allow programmers to prompt the system for functionality; this code is generated based on the current programming context as well as the prompt/request.

What is generated is not only plausible-looking code, it is often reasonably performant: XX demonstrated that general-purpose LLM can solve well-articulated university-level programming problems. At the same time, general-purpose LLMs can provide explanations about error codes and compiler messages. Furthermore, programmers can formulate questions to ask the LLM about potential solutions to programming errors or mistakes. Researchers have demonstrated that these explanations or suggestions can be helpful to programmers.

At the same time, LLMs are not fool-proof. When faced with ill-formed prompts, an LLM will still attempt to generate a plausible response; many times, these plausible responses are not as effective. For instance, it may not error-check properly, or fail in certain test cases that were not articulated by the programmer.

To some extent, these challenges can be mitigated through the use of ``prompt-engineering'', or by engineering meta- prompts that recursively pass the results back into an LLM to generate a better response. In XX, XX show that subtlely modifying the prompt to use ``XXX'' phrase as opposed to ``YYYY'' results in generated code being correct XX more of the time. This type of prompt engineering is a common approach, but requires considerable hand tuning, and it is unclear whether results will continue to have long-term benefit as newer general-purpose LLMs are trained. Another approach to improve the code generated by LLMs involves the use of meta-prompts that recursively examine code previously generated by an LLM. For example, XX demonstrated that it is possible to ask an LLM to critique an earlier response, and then to generate a better response based on this critique. While we expect techniques for ameliorating poorly formed prompts, these tools are still generally formulated for, and designed for programmers to use. It is unclear how non-programmers might use these tools to generate code (or, in practice, to form or articulate their needs), and how LLMs will respond to these requests. Our work aims to address this gap.

\subsection{Interactive Spaces}

To circumscribe our exploration, we focus on interactive spaces such as those found in 

\end{comment}



%    \item \textit{Progressive refinement will be common, as will feedback from the user.} Although our elicitation study itself does not capture this in the raw data, participants made clear that they expected the system to regularly make mistakes, and that one of their desired modes of interaction would be to correct the system as the interaction went on. This suggests that while it would be valuable for the agent to correctly generate something at the outset, users seem to be aware that this may not always go well, and that they will need to progressively refine the scene through clarifications.
    

05 system.tex


\subsection{Design Vision}

With Oastaad, the intention was to democratize the design of VR scenes: to enable people who may not have a programming or technical background to fashion virtual environments. Following on prior work, our goal was to simplify how scenes could be designed---rather than designing scenes in desktop based tools, which would require additional training on visual coding, textual coding, 3D scene management and so on, our goal was to enable people to design scenes by describing them. Our intention was to replace technical coding with verbal language and embodied interaction.

Such descriptions of scenes and environments are common. For example, if one were to describe how one's living room were set up, it is common to employ embodied storytelling---gesturing at the placement of imaginary objects or outlining the shape, location or orientation of objects (e.g. ``The couch is over here along the wall, and it faces a coffee table that has a flower pot on it.''). One might use such storytelling techniques to describe a funny incident (e.g. ``Johnny put his glasses here, which you cannot see from the couch, so he thought he lost his glasses.''). Our intention was to use such descriptions as a basis for driving Oastaad, a programming agent, that could respond to similar kinds of descriptions to design a virtual environment.

This type of embodied storytelling relies on both diectic references (e.g. a pointing gesture accompanying, ``I like this chair''), as well as body movements (e.g. head orientation or movements). Such proxemic information would be commonplace for a person to interpret another's embodied interactions with the space---for instance ``The couch goes over here,'' (spoken while pointing, and looking at the wall). This point then, our goal was to allow users to inhabit the space they were designing, rather than describing and designing the scene from an omnipotent view. Our expectation was that this would allow them to iterate and refine their ideas as they saw them realized by the programming agent at scale, and in an embodied way.

%    The Tasker is supplied information about the user's position in the scene, and what objects are in their field of view.
%- Preconceived Notions such as available 3D prefabs, actions, and triggers.

%- SceneManager details objects currently in the scene, their quantity, which ones are within the field of view, and their position relative to the user. This is not always essential, but it is included as it helps in reducing random outputs.

%The JSON output from Tasker comprises two primary components. The message determines the necessity of code, requests further information or clarification from the user if needed, or provides a straightforward interpretation of the user's request and a set of clear, actionable tasks akin to pseudo-code.

%Tasker's operation involves two distinct functions:

%1. Object and Action Identification: It identifies specific objects and actions mentioned in the prompt, using all the provided information. In cases of ambiguity or if the referenced object is not in the database, Tasker may seek more details from the user, acknowledge the request's unfeasibility, suggest alternatives, or note execution limitations.

%2. Task Generation: After clarifying the user's intent, Tasker formulates a sequence of tasks for the next module. This involves breaking down the prompt into specific, actionable tasks, such as object creation, modification (e.g., illumination, resizing), and setting up triggers for interactive behaviours.



%The main role of the Tasker is transforming user prompts into structured tasks, and providing the coder module with directives that are easily interpretable by computers to facilitate better code generation.
    % The main role of Tasker is to convert the user's natural language prompt into a set of programming tasks for the next module. This module uses both the user's prompt, as well as an understanding of the current scene hierarchy (i.e. what objects are in the scene, how they are arranged), as well as a description of the user's position and orientation in the world. This module performs two fairly distinct tasks: (1) it determines which objects are being referred to in the scene and/or which objects should be instantiated given the prompt, and (2) it develops a programming plan for the subsequent module.

    % This subsystem determines which objects may be being referred to in the prompt. This subsystem accounts for what the user sees and may be pointing to, as well as what objects are currently in the scene. For example, in Figure ~\ref{fig:normal-referent}(c), it would determine first whether a lamp existed in the environment, and if so, \textit{which} lamp would need to be turned on. This subsystem also finds substitutes in the system for objects, allowing users to use synonyms for scene objects. In Figure ~\ref{fig:normal-referent}(c), the user could have referred to the ``light'' or ``table lamp'' and so on. Finally, if there are multiple possibilities for objects being referred to, the system chooses objects that are within view, and closest to the center of the user's viewing angle.

    % Second, the subsystem breaks down natural language prompts into smaller programming tasks. For instance, the natural language prompt in Figure ~\ref{fig:normal-referent}(b) (``Create a desk with a lamp on it'') would be broken down into two tasks, involving the instantiation of both a desk and a lamp, and then placing the lamp atop the desk. The system also generates logical completions for prompts. The prompt in Figure ~\ref{fig:normal-referent}(d) (``Make the lamp turn on when I touch it'') would get turned into two tasks: one to turn on the lamp when it is touched; another to turn the lamp off when it is no longer touched.

    % Plans generated by this subsystem are natural language, and used as input for the Coder.

    %\item[\texttt{Coder}] The Coder is an advanced generative AI agent specifically designed to produce C# code in response to user prompts. Its primary function is to translate a list of tasks, generated by the Tasker module, into executable code blocks. These tasks are essential for achieving the user's specified goals. The Coder interacts with two key APIs: SceneManagerAPI which manages the scene as a whole and has information such as the hierarchical structure of objects, information about the room, walls, and the state of the user, and ObjectAPI, which manages individual object properties, tracking their state and the range of possible actions associated with each.

    %Similar to the Tasker, the Coder's output is structured in JSON format, encompassing two main components. The first is a series of named code blocks (methods/functions), each with a natural language description. This format aids in storage and retrieval of code when a future prompt has the same task, and also informs users to understand how their prompt is being executed/coded. The second component is the source code, serving as the input for the next module in the workflow.

     %The coder's operation can be summarized into two primary functions:
     
     %1. Creation of Code Blocks per Task: First, it looks at each task separately and generates individual blocks of C# code for each task provided by the Tasker Module. Each block is crafted to accomplish a specific task and is accompanied by a descriptive commentary in natural language to facilitate understanding and future reference.
     
     %2. Creating a Comprehensive Code: The second function involves synthesizing these individual code blocks into a cohesive source code. This comprehensive code connects all the tasks to cover the user's full objective.

     
    %Similar to the Tasker, the Coder's output is structured in JSON format, encompassing two main components. The first is a series of named code blocks (methods/functions), each with a natural language description. This format aids in storage and retrieval of code when a future prompt has the same task, and also informs users to understand how their prompt is being executed/coded. The second component is the source code, serving as the input for the next module in the workflow.

     %The coder's operation can be summarized into two primary functions:
     
     %1. Creation of Code Blocks per Task: First, it looks at each task separately and generates individual blocks of C# code for each task provided by the Tasker Module. Each block is crafted to accomplish a specific task and is accompanied by a descriptive commentary in natural language to facilitate understanding and future reference.
     
     %2. Creating a Comprehensive Code: The second function involves synthesizing these individual code blocks into a cohesive source code. This comprehensive code connects all the tasks to cover the user's full objective.

          %Each change, along with its explanation, is dynamically integrated into the running virtual reality (VR) scene in real-time (``hot'' injection). 



\begin{comment}
\begin{figure}
  \caption{Ostaad}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/images/Ostaad.png}
\end{figure}
\end{comment}


%Some examples of errors are apparent language issues, the use of API/functions that were non-existent, and the creation of the wrong or non-actionable output.





06 conclusions and future work.tex

%This type of embodied storytelling relies on both diectic references (e.g. a pointing gesture accompanying, ``I like this chair''), as well as body movements (e.g. head orientation or movements). Such proxemic information would be commonplace for a person to interpret another's embodied interactions with the space---for instance ``The couch goes over here,'' (spoken while pointing, and looking at the wall). This point then, our goal was to allow users to inhabit the space they were designing, rather than describing and designing the scene from an omnipotent view. Our expectation was that this would allow them to iterate and refine their ideas as they saw them realized by the programming agent at scale, and in an embodied way.
